RecSys Arena: Pair-wise Recommender System Evaluation with Large Language Models

Evaluating the quality of recommender systems is critical for algorithm design and optimization. Most evaluation methods are computed based on offline metrics for quick algorithm evolution, since online experiments are usually risky and time-consuming. However, offline evaluation usually cannot fully reflect users' preference for the outcome of different recommendation algorithms, and the results may not be consistent with online A/B test. Moreover, many offline metrics such as AUC do not offer sufficient information for comparing the subtle differences between two competitive recommender systems in different aspects, which may lead to substantial performance differences in long-term online serving. Fortunately, due to the strong commonsense knowledge and role-play capability of large language models (LLMs), it is possible to obtain simulated user feedback on offline recommendation results. Motivated by the idea of LLM Chatbot Arena, in this paper we present the idea of RecSys Arena, where the recommendation results given by two different recommender systems in each session are evaluated by an LLM judger to obtain fine-grained evaluation feedback. More specifically, for each sample we use LLM to generate a user profile description based on user behavior history or off-the-shelf profile features, which is used to guide LLM to play the role of this user and evaluate the relative preference for two recommendation results generated by different models. Through extensive experiments on two recommendation datasets in different scenarios, we demonstrate that many different LLMs not only provide general evaluation results that are highly consistent with canonical offline metrics, but also provide rich insight in many subjective aspects. Moreover, it can better distinguish different algorithms with comparable performance in terms of AUC and nDCG.

==> content/discussion.tex <==

\subsection{Absolute evaluation and relative evaluation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{samples/figures/score-1.png}
    \caption{The Differences Among Offline Metric (AUC), LLM-based Pair-wise Evaluation Reaults (Q), and LLM-based Absolute Evaluation Score \label{fig:absolut_score}}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{samples/figures/score-2.png}
    \caption{Absolute score \label{fig:absolut_score}}
\end{figure}




\subsection{Future Works}
% \textbf{Future works:} 
Our experiments have demonstrated that the evaluation framework based on LLM is capable of conducting accurate and interpretable assessment of recommendation quality. There are some possible directions to further improve the LLM-based evaluation framework.
First, since factors influencing user clicks may involve environmental factors such as location and time in addition to user preferences, in the future, we could incorporate environmental factors into the evaluation framework and design a context-aware evaluation method. The feasibility of this approach lies in the fact that some datasets (e.g.,) include the attribute of timestamps.
Second, currently, large language models can only perform user-centric evaluations. During a single interaction, a large language model can only role-play as one user and is unable to see information and recommendations for other users, meaning it cannot view the full picture of the entire test set. In the future, we could consider how to use large language models for system-centric evaluations, such as grouping users and evaluating them as a group.
Third, due to the limited coverage of knowledge within large language models, there may be a reduction in the effectiveness of evaluating long-tail items or niche user groups.
Fourth, to enable large language models to utilize more recommendation-related knowledge during the evaluation process, we plan to fine-tune the evaluation model with supervised learning using recommendation data in the future.
